MICDIR: Multi-scale Inverse-consistent Deformable Image Registration using UNetMSS with Self-Constructing Graph Latent

Image registration is the process of bringing different images into a common coordinate system - a technique widely used in various applications of computer vision, such as remote sensing, image retrieval, and, most commonly, medical imaging. Deep learning based techniques have been applied successfully to tackle various complex medical image processing problems, including medical image registration. Over the years, several image registration techniques have been proposed using deep learning. Deformable image registration techniques such as Voxelmorph have been successful in capturing finer changes and providing smoother deformations. However, Voxelmorph, as well as ICNet and FIRE, do not explicitly encode global dependencies (i.e. the overall anatomical view of the supplied image) and, therefore, cannot track large deformations. In order to tackle the aforementioned problems, this paper extends the Voxelmorph approach in three different ways. To improve the performance in case of small as well as large deformations, supervision of the model at different resolutions has been integrated using a multi-scale UNet. To support the network to learn and encode the minute structural co-relations of the given image-pairs, a self-constructing graph network (SCGNet) has been used as the latent of the multi-scale UNet - which can improve the learning process of the model and help the model to generalise better. And finally, to make the deformations inverse-consistent, cycle consistency loss has been employed. On the task of registration of brain MRIs, the proposed method achieved significant improvements over ANTs and VoxelMorph, obtaining a Dice score of 0.8013 \pm 0.0243 for intramodal and 0.6211 \pm 0.0309 for intermodal, while VoxelMorph achieved 0.7747 \pm 0.0260 and 0.6071 \pm 0.0510, respectively

==> sections/x_2_related_work.tex <==
\subsection{Related Work}
\label{ch:relatedwork}

We begin our discussion by discussing the paper by \cite{de_vos_deep_2018}. Authors of this literature, described, pretty much comprehensively, the ideas behind medical image registration system and the ways to evaluate this. Unlike their predecessors, \cite{de_vos_deep_2018} focused on unsupervised learning whereby registration is done by optimising a loss function. A ConvNet was used here to derive a function like parameter set, which was later used to register the moving image in one-shot.

They started their literature by showing arguments in favour of using deep learning (DL) techniques for medical image registration. They argued about the capacity of DL techniques for automatically extracting the relevant features. They also argued about the qualities of convolutional architecture and deep learning in general like parallelisability and robustness. Following this discussion, they emphasised the necessity of going unsupervised in the field of medical image registration. They argued the drawbacks of supervised methods by mentioning the necessity of manual annotations or artificial synthesisation of training examples, which can be difficult to obtain and time consuming to produce. On the other hand, unsupervised techniques do not suffer from these issues. 

Bearing these issues in mind, de Vos et al. proposed to calculate a dense displacement vector field (DVF) between the moving and the fixed image. In order to achieve this DVF, they, instead of directly optimising a set of parameters, used CNNs weights as parameters of the DVF and optimise those to calculate the transformation parameters. Thus, the task of the CNN becomes to detect and utilise the similarity in the fixed and the moving image to understand the parameters of the registration.

VoxelMorph, as proposed by \cite{balakrishnan_voxelmorph_2019}, is another significant literature that many of the later implementation considered to be a baseline for comparing their implementations. One of the main differences between VoxelMorph and \cite{de_vos_deep_2018} is the way they are inputting the image into the architecture. While de Vos et al. takes two separate inputs, one for moving and another for fixed, and process both of them parallelly, VoxelMorph concatenates them and process them together. 

However, authors of VoxelMorph begins their discussion by identifying the shortcomings of traditional registration methods that considers pairwise optimisation of moving and fixed images through the alignment of the voxels with similar appearances. But these require higher computational power which makes them difficult to use for real-time test cases. To alleviate this issue, VoxelMorph proposes two alternatives: the first one deals with input volumes and registration field calculated by the CNN based architecture and the second one utilises anatomical segmentations. The authors focused on 3D volumes of single channel (grayscale). They designed a CNN based network that is used to parameterise the displacement field u between the fixed and the moving image. 

The next literature that inspired us is from \cite{tang_admiraffine_2020}. They proposed an end-to-end image registration method with three components, namely the affine registration module, the deformable registration module, and the spatial transformer module. 

They initiated their discussion by pointing out the drawbacks of traditional optimisation based registration processes: they emphasised on the speed of these methods and their inability to handle complex structures. Following this discussion, they stated some of the limitations of the supervised algorithms, e.g the need for labelled ground-truths, etc. These arguments made the ground for the necessity of unsupervised approach to tackle medical image registration. They acknowledged the contributions of \cite{jaderberg_spatial_2016}, \cite{de_vos_deep_2018}, and \cite{balakrishnan_voxelmorph_2019} and drew inspiration from these. However, they mentioned about the necessity of pre-aligned data for training these unsupervised approaches. To mitigate these challenges, \cite{tang_admiraffine_2020} proposed their system as an end-to-end solution for registering an image. 

In order to realise such a solution, ADMIR learns, by employing a ConvNet, 12 parameters related to affine transformation. For the deformable transformation, they introduced a ConvNet that is capable of learning the displacement vector field (DVF). They have used Spatial Transformation modules after each of these transformation parameters are learned. They have used a compound loss function which is composed of three individual loss entities: the first loss is calculated between the affinely transformed image and the fixed image, the second one is calculated between the fully warped image and the fixed image, and the last one is calculated as the smoothness loss. One notable distinction between \cite{de_vos_deep_2018} and ADMIR is the concatenation of fixed and moving images, instead of feeding them to separate channel. The same approach was followed by \cite{balakrishnan_voxelmorph_2019}. 

On the other hand, CycleMorph, due to \cite{kim_cyclemorph_2020}, provided an intuitive solutions to image registration problem. They argued that the existing deep learning based solutions, in most cases, are unable to preserve the topology of the image, resulting in an unwanted degeneracy problem. To mitigate this issue, they used cycle consistency to regularise the diffeomorphism generated by the model. In order to realise their effort, they are generating two diffeomorphic deformation vector field, the first of these takes an image and generates a deformed version of it, this version is then gets propagated to the next network, whereby another network then do the inverse and generates the original image out of this deformed one. Both of the network is updated and optimised using the same loss function. Thus, cycle consistency is used as a constraint that regularises the deformation vector field, so that it doesn't generate unrealistic image folds which cannot be reverted back to the original image. Furthermore, this paper also proposes a multiscale image registration technique that uses global and local registration methods to optimise the usage of GPU while processing massive dataset.

Loss function that was used here in this paper, has three components. First of them is the registration loss, in which local cross-correlation was used as similarity function for it's less sensitive nature to the contrast variation. In addition to this, an l2 regulariser was also used to make the deformation field smooth. The second part is the cycle loss, in which l1 norm was used to ensure cycle consistency. Apart from these two, a novel loss function was introduced here that is the identity loss. The rationale for this is: stationary regions of images should not be changed. Identity loss ensures this property. For evaluation, Jacobian matrix was produced to evaluate the diffeomorphic performance of the deformation. Furthermore, Dice coeffiecient and target registration error was used. On the flip side, this approach requires manually delineated anatomical structures and manually indicated landmarks for evaluation of the registration performance, which introduces the risk of human error.

A similar idea was used by \cite{zhang_inverse-consistent_2018}. He utilised inverse consitency and prepared a pipeline in unsupervised fashion for deformable image registration. In this approach, he took a pair of images and ensured that those are symmetrically deformed toward each other. In order to facilitate the production of realistic image, he introduced an anti-folding constraint and smoothness constraints that restricts the amount of folds in the warped image and ensures the smoothness of the produced image, respectively. In the beginning of the pipeline, the author used two fully connected layers (FCN) to create two non-linear, dense transformation of the input images. This FCN is a U-net style network with varying filter and sampling sizes. These two FCNs share their parameters. Output of these two FCNs are two discrete displacements fields that Zhang \cite{zhang_inverse-consistent_2018} labelled as Flow. This flow is then fed to an inverse network and a grid sampler. The grid sampler produces a warped image. On the other hand, to implement the inverse consistent constraint, the author designed an inverse network that takes the discrete displacements fields and the negative of it and adds them together. Thus, by combining two such flow fields from two FCNs, using L2 norm, ICNet calculates the inverse constraint. 

However, \cite{dalca_unsupervised_2019} realised that all of these methods considered point estimates of the weights, leaving probabilistic framework aside. They argued that classical registration methods had a rigorous theoretical background, but lacked in speed as they were built to work with pairs of images individually. On the other hand, recent methods, developed in deep learning based models, are much faster, but they lack the theoretical background. \cite{dalca_unsupervised_2019} attempted to bridge the gap by utilising a probabilistic deep learning method that utilises registration uncertainty. In addition to this, they ensured the diffeomorphic properties of the registered image which is able to preserve topological information. They modelled the registration problem as a variational inference on probabilistic generative model. To realise this concept, they utilised a CNN-based model with a combination of upsampling and downsampling, configured to match the GPU setup. The end-to-end system takes two inputs, one moving 3D image and one fixed image, both of which run through the aforementioned CNN network, giving an output of two: the mean and variance of the associated velocity field. These two parameters builds the velocity field that then pass through an integration layer built using squaring and scaling operations. This layer produces a deformation field which is used by a spatial transformer to produce the final moved image. However, because of the probabilistic nature of their algorithm, they had to decide how to solve the intractability issue of the computation of posterior probability for the parameters; they solved it using variational approach and proposed to calculate an approximation of the posterior probability instead of being exact. 

\cite{khawaled_unsupervised_2020} took a different approach for solving the image registration problem probabilistically. Instead of approximating the posterior probability using some variational method, \cite{khawaled_unsupervised_2020} chose to model the true posteriori using Stochastic Gradient Langevin Dynamics (SGLD) method, as proposed by \cite{welling_bayesian_nodate}. In this method, a small amount of noise is purposefully injected during the training of the mini-batch stochastic gradient descent, to guide the descent to a point that is equivalent to sampling from the true posterior distribution. That way, we don't have to work with an approximation, rather we can have the true distribution parameters. 

Khawaled et al. argued in favor of the bayesian treatment of image registration problem because of the small size of the dataset. They argued that this problem alone can cause overfiting if point estimates are used, instead of probability estimates.

On the other hand, \cite{hansen_tackling_2020} expressed their concern over the sub-standard perfomance of deep learning techniques in case of inter-patient abdominal MRI or CT of lungs during breathe-in and breathe-out phase. They blamed the use of encoder-decoder style architecture, U-net style architecture to be precise, for this. They argued that U-net architectures perform poorly in case of very large deformations, even if multiple levels of encoding-decoding is used. To mitigate this, they proposed to calculate the displacement vector field directly from the two input images. They utilised a CNN based feature extractor that is able to extract features of interest from the images. But they don't capture all the features in order to generate a vector field, rather they choose a set of key points where they focused their extraction process. They have selected these points based on Foerstner interest operator. Thus, they created a feature map in a low dimensional space that they call displacement map. This map then generates the moved image. The flip side of this method is the usage of fixed points to extract they features. Some of the important features can easily get missed because of this selection process.

\cite{grigorescu_diffusion_2020}, on the other hand, argued in favour of combining structural and microstructural information. They argued that, from the point of tracking the microstructural changes, it is even better to combine structural information, obtained from T2-weighted images, and microstructural information, extracted from diffusion tensors. Such an approach makes the process faster to an extent that registration can take place in one pass only. In order to achieve that, they have based their model on VoxelMorph, due to \cite{balakrishnan_voxelmorph_2019}, and added layers on top of this which are capable of handling diffusion tensor images. Initially, the took a pair of fixed and moving T2 weighted images and combined them together to feed into a CNN based extractor that extracts a velocity field by calculating the displacement of voxels. This then is followed by a topology-preserving scaling and squaring layer that gives the dense displacement field (DDF). This DDF is the used to spatially transform and warp the moving image into a moved image. 

\cite{qin_biomechanics-informed_2020} worked with for developing the way we regularise neural networks for image registraion problem. They identified that even if current regularisers are capable of making this image registration problem a well-posed problem, from an ill-posed one, these are unable to incorporate domain specific information. Furthermore, these regularisers often make generic assumption, which might become counter-productive. To alleviate these issues, \cite{qin_biomechanics-informed_2020} proposed a bio-mechanic informed regulariser that incorporates domain specific information which in turn will help immensely in producing much more realistic images as the regulariser itself is more realistic than some generic one like smoothness constraint, etc. To realise this, the authors utilised a variational auto-encoder (VAE) that learns the bio-mechanically possible deformations. To be more precise, biomechanical simulations, done by partial differential equations, are run to simulate possible deformations. This simulation are then run through a variation auto-encoder which gives the probability of these simulations. This learnt VAE can then used as the regulariser for any registration network. 

==> sections/x_3_analysis.tex <==
\section{Methods}
\label{ch:methods}

\subsection{Direct Optimization based Methods}
\subsubsection{Gradient Descent based Technique}
\subsubsection{Introduction}
In the previous sections we have seen parameterizing a function using large deep learning models to calculate deformation fields. We also have discussed its advantages against traditional iterative algorithms in terms of performance and speed. In current method, we ditch the usage of deep learning model and optimize the deformation field directly using gradient descent without any model parameters. The rationale behind direct optimization is to experiment on registration performance without any deep learning model or complex mathematical optimization procedure. \cite{Fuse2000ACS} describes various techniques based on gradients to estimate optical flow, \cite{Sherina2020DisplacementFE} discusses using multi-scale, iterative, numerical approaches and using additional speckle information to solve registration problem.

\subsubsection{Training Procedure}
Our focus in this experiments is to directly optimize a deformation field of size \( 3 \times 128 \times 128 \times 128 \) for a pair of images using image similarity metric such as NCC or NMI and smoothness loss. Equation \ref{eq:direct_optimzation_loss} explains the loss function used to optimize the deformation field. \(f \) and \(m \) represents fixed and moving image, \( l_{sim_{m->f}} \) represents similarity loss and \(l_{sm_{m->f}}\) represents smoothness loss to regularize deformation field. \(\alpha\) and \(\beta\) We experiment using various optimizers with default settings in Pytorch \cite{NEURIPS2019_9015}, 1500 epochs and report the result for the same evaluation dataset as used for other deep learning based methods. 


\begin{equation}
l_{total} =  \alpha(l_{sim_{m->f}})  + \beta(l_{sm_{m->f}}) 
\label{eq:direct_optimzation_loss}
\end{equation}

\subsection{Deep Learning based Methods}
\subsubsection{ICNet} 

\subsubsection{Introduction}
 \cite{zhang_inverse-consistent_2018} are performing image registration both ways, i.e. Let's assume one image as A and another as B, with ICNet architecture image A is registered to image B and called as warped\_A and image B registered to image A is called as warped\_B. When image A gets registered to image B, in the process a flow or displacement vector field named as Flow\_AB is defined. Similarly, when image B will get registered to image A, flow Flow\_BA will be generated.  \cite{zhang_inverse-consistent_2018} has denoted registered or warped images as warped\_A and warped\_B.  

\subsubsection{Architecture}
ICNet's \cite{zhang_inverse-consistent_2018} architecture consists of a fully convolution network that takes as input image A and B and results in warped\_A and warped\_B by modeling Flow\_AB and Flow\_BA. Authors have proposed two modules of fully convolution network for registering, one for image A to B, B being the target image and another one for image B to A, A being the target image. These two FCN modules share parameters and have the same structure. The fully convolution network architecture used in \cite{zhang_inverse-consistent_2018} paper is UNet \cite{iek20163DUL} \cite{Ronneberger2015}. This network comprises of two paths - the contracting path used for an image's under-sampling and for oversampling of an image - an expanding path. 

The ICNet \cite{zhang_inverse-consistent_2018} pipeline consists of a grid sampler that takes as input image A and flow Flow\_AB and gives out warped\_A. Similarly, image B and flow Flow\_BA as inputs result in warped\_B as the output. A grid sampling network is nothing but a spatial transformer network \cite{jaderberg_spatial_2016} that is fully differentiable. It consists of a generator that generates a spatial grid and a sampler. This spatial grid gets converted to a sampling grid by using the flow or dvf which we get from the fully convolution network. Finally, the source image is warped by making use of the sampling grid by the sampler. 
Authors \cite{zhang_inverse-consistent_2018} made use of bilinear mode for interpolation. Architecture of ICNet is described in \ref{fig:ICNet Overview}

\begin{figure*}[!htb]\centering
    \centering
    \includegraphics[width=1.01\textwidth]{figs/icnet_architecture.png}
    \caption{ICNet Overview}
    \label{fig:ICNet Overview}
\end{figure*}

\subsubsection{Training}
ICNet \cite{zhang_inverse-consistent_2018} proposed three types of constraints, inverse consistent constraint, antifolding constraint, and smoothness constraint. Inverse consistent is a regularisation term used for penalizing the deviation of the transformation fields (flow) from their corresponding opposite or inverse mappings i.e. inverse flow. The second constraint \cite{zhang_inverse-consistent_2018} mentioned is the antifolding constraint that is to prevent folding from happening in the flow generated. The last constraint used is the smoothness constraint. This constraint encourages the local smoothness of transformation fields.  For the objective function, \cite{zhang_inverse-consistent_2018} used mean squared distance for measuring the similarity between the fixed image and the registered image. So, the final objective function becomes the sum of similarity, inverse consistent, antifolding, and smoothness constraint, where the constraints are multiplied by hyperparameters a,b and c respectively to balance out their values. 


\subsubsection{FIRE} 
\subsubsection{Introduction}
\cite{Wang2019} talks about unsupervised image registration for intermodality. This method does multi-modal registration for any dimension of the image, to achieve this, it makes use of cycle consistency loss and inverse consistent property. In this paper, \cite{Wang2019}, similar to ICNet \cite{zhang_inverse-consistent_2018} both image A and image B gets registered to each other. The model designed gives two fields that is used to register image A to B and image B to A. These transformation fields are achieved by minimizing the objective function. 

\subsubsection{Architecture}
FIRE's \cite{Wang2019} architecture consists of total 5 components. First is an encoder which is used for extracting features that are not modality dependent, then comes two decoders, which are used for mapping the attributes extracted by the encoder with the warped images. And lastly, two transformation networks are used for generating transformation fields. During the registration process, the encoder's output is also warped to the transformation field. 

We have first defined a residual block or a resnet block according to \cite{hara3dcnns} and used this resnet block in encoder and decoder networks.
Encoder's architecture consists of 1 convolution layer followed by two layers of downsampling and then there are 4 residual blocks. Whereas, in the decoder network, we first have 4 of the residual blocks, then comes two oversampling convolutional layers where we have have used 3D transposed convolution operator and then final convolutional layer along with a 1D convolutional layer. Kernel size for the convolutional layers is 3 and we have used instance normalization as defined in paper \cite{Wang2019} and leaky relu as the activation function. 

In the fire paper, \cite{Wang2019} for generating transformation field, authors have made use of both affine as well as deformable transformation networks. But we have used already affine registered images (i.e T1 affinely registered to T2 and T2 affinely registered to T1), hence we are exploring only deformable network in this case. For deformable transformation network, there are two convolutional layers that intakes encoded image x and image y respectively and then activation function leaky relu is used. These two layers are then concatenated and passed to a residual block followed instance normalization, leakyrelu, convolutional layer and again instance normalization and finally tanh. All of these extracted attributes result in a displacement vector field. This field is then passed to a grid sampler or a spatial transformation network \cite{jaderberg_spatial_2016}. Architecture of FIRE is described in \ref{fig:FIRE Overview}

\begin{figure*}[!htb]\centering
    \centering
    \includegraphics[width=1.01\textwidth]{figs/fire_architecture.png}
    \caption{FIRE Overview}
    \label{fig:FIRE Overview}
\end{figure*}

\subsubsection{Training}
The objective function for this network has three components, the first is synthesis loss, the second one is registration loss and the last is a regularization term. 
Synthesis loss \cite{Wang2019} again has four parts, the first is accuracy loss, the second one is for the features extracted, next is the loss for cycle consistency for the intermodality synthesis and lastly is the alignment loss. 
Registration loss consists of two losses, the first is accuracy loss for the registration and then a loss function for inverse consistency. All of these components for synthesis and registration loss makes use of the Root Mean Square error function. The regularization term in the original paper has three terms, we are not considering the first two terms - synthesis regularization and registration regularization as both of them make use of affine network output and we are already feeding the network affinely registered images. The third component of regularization is a smoothness constraint which is calculated by non-rigid transformation fields to the smooth loss function and summing and multiplying it with a hyperparameter. Value of this hyperparameter or scaling parameter \cite{Wang2019} (let's say a) is calculated as - 

\begin{equation}
   a = (2^2^m) / (10M)
\end{equation}

where m stands for the dimension of the images (3 in our case) and M represents the number of pixels in the image. (128 or 64 in our case).




\subsubsection{ADMIR} 
ADMIR \cite{tang_admiraffine_2020} (Affine and Deformable Medical Image Registration) is an affine and deformable image registration that works end to end. This uses the convolution neural network (ConvNet) to perform unsupervised image registration. This method doesn't require the images to be pre-aligned, which in turn helps to do image registration quickly with good accuracy. 

An affine registration network, a deformable registration network, and a spatial transformer are the three fundamental components of ADMIR. Both Affine and Deformable networks were trained at the same time in the original publication. The traditional image registration techniques improve the registration by iteratively optimizing the similarity function. However, these are time-consuming and incapable of dealing with complex shape changes. ADMIR made an effort to decrease time while simultaneously improving the quality of registration results. We know that getting labelled data is always not easy. The ADMIR tries to solve this problem as it is an unsupervised learning algorithm, which means our data need not be labelled with information like landmarks, ground-truths, or pre-known transformations. 

ADMIR \cite{tang_admiraffine_2020} has two sub-networks, one focuses on affine registration and the other one focuses on deformable registration. The fixed and moving pictures are concatenated and sent into the Affine ConvNet, which predicts 12 affine transformation parameters (rotation, translation, scaling, and shearing) that are used to calculate the DVF $u_a$, which is then used by the spatial transform to coarsely warp the moving image. The coarsely warped and fixed images are then combined and fed into the Deformable ConvNet, which calculates the DVF $u_d$.  To get the final registration result, the final DVF $u_f$ is calculated by aggregating DVF $u_a$ and DVF $u_d$ with the help of a spatial transformer, which warps the moving image to fully register the moving and fixed images.

We tried to do the end-to-end affine registration with all the modules as mentioned in the ADMIR \cite{tang_admiraffine_2020}. However, we did not get good results as the affine registration module did not produce the desired output. So, we reverted to the usual preprocessing pipeline that we are using in this paper with the help of ANTS and Freesurfer, and then we used the deformable module of ADMIR to perform registration. This also allows us to perform aggregation of DVFs. We have changed the loss function as we were not using the affine module.

Firstly, to obtain the local difference between the two images, the fixed and moving images are first concatenated and then input into the deformable network. The deformable network contains encoder and decoder stages. The encoder stage contains a stack of convolutional and strided convolutional layers to lower the spatial dimension step by step, allowing the network to learn local similarity from features with varied resolutions. Similarly, the Decoder Stage contains successive deconvolutional and convolutional layers, allowing the network to restore the low-resolution feature to the same resolution as the input image. 

As mentioned in ADMIR \cite{tang_admiraffine_2020}, We do element-wise addition of two features between two same-size cubes to make maximum use of the information in low- and high-resolution features. This in turn connects to a final fully convolutional layer which determines the final DVF. The final DVF is used by the spatial transformer to fully register the moving image to the fixed image. After each convolution operation, LeakyRelu and Batch Normalization are utilized, except for the final convolutional layer. 

Each convolution block is made up of a strided convolutional layer with a kernel size of 3 × 3 × 3 and a stride of 2 and 1 for the decoder and encoder, respectively. A Batch Normalization layer and a LeakyRelu activation layer are also added after each layer. We changed the loss function a little because we aren't utilizing the affine module. As indicated in the paper, we employed gradient loss for smoothness in addition to normalized cross-correlation (NCC) as a similarity loss.


\subsubsection{Voxelmorph}
\subsubsection{Introduction}
Voxelmorph \cite{balakrishnan_voxelmorph_2019} is a deep learning based, unsupervised, pairwise, deformable registration framework. The framework aims to use CNN for parameterizing the function to calculate deformation field. The model is unsupervised and learns based on image similarity metric, Hence it does not require costly supervision and generation of deformation field for training. The framework also incorporates additional supervised segmentation training regimen that could help further improve the performance on the dataset. Traditional iterative approaches have the disadvantage of optimizing deformation field for each pair of images independently of others and takes minutes to compute on GPU. Voxelmorph takes in two n-D volumes and compute deformation field in few seconds. This reduces compute time whilst maintaining performance. An overview has been shown in below Fig \ref{fig:Voxelmorph Overview} \cite{balakrishnan_voxelmorph_2019}
\begin{figure*}[!htb]\centering
    \centering
    \includegraphics[width=1.01\textwidth]{figs/voxelmorph_overview.png}
    \caption{Voxelmorph Overview}
    \label{fig:Voxelmorph Overview}
\end{figure*}

\subsubsection{Model}
Voxelmorph is based on UNet \cite{iek20163DUL} and has a similar encoder, decoder based blocks with skip connections. Voxelmorph takes a single input of concatenated moving and fixed image. Each encoder block halves the spatial dimensions using strides of 2 and applies non linear activation LeakyReLU with parameter \(0.2\). As we reduce the feature dimensions subsequent encoders learn more high level information about the images. The decoder block consists of an upsampling block that upscales the feature dimensions by a factor of 2 and convolution layer that concatenates the corresponding encoder features to upsampled features and applies convolution on them. This is finally fed to few convolution layers that maintains the spatial dimensions of the deformation field and captures of finer changes in anatomy. Fig \ref{fig:Voxelmorph Architecture} \cite{balakrishnan_voxelmorph_2019} shows the architecture of Voxelmorph.
\begin{figure}[!htb]\centering
    \centering
    \includegraphics[width=1.0\textwidth]{figs/voxelmorph_architecture.png}
    \caption{Voxelmorph Architecture}
    \label{fig:Voxelmorph Architecture}
\end{figure}

\subsubsection{Training Procedure} The dataset comprises of T1 3731 brain volumes from publicly available dataset, it consists of both healthy and diseased person of varied age distribution. The volumes are preprocessed using Freesurfer \cite{Fischl2012FreeSurfer}. Scans were resampled to standard \(256 \times 256 \times 256\) with 1mm isotropic size. The scans are then removed of bias fields, skull stripped and affine registration applied. After visual inspection few of the bad preprocessed scans are rejected. The affinely registered volumes are fed into the network and the resulting deformation field is used to transform moving image using Spatial Transformer \cite{Jaderberg2015SpatialTN}. The warped image is then compared against the fixed image using a similarity metric such as MSE and NCC. The deformation field is regularized using a smoothness loss function that penalizes unrealistic sharp deformations. Equation \ref{eq:unsup_loss} shows the overall loss function where \(f\) is fixed image, \(m\) is moving image, \(\phi\) is the deformation field and \(\mathcal{L}_{sim}\) is the similarity loss, \(\mathcal{L}_{smooth}\) is the deformation field smoothness loss, \(\lambda\) acts as hyperparameter for regularization term.
\begin{equation}
    \mathcal{L}_{us}(f, m, \phi) = \mathcal{L}_{sim}(f, m \circ \phi) + \lambda\mathcal{L}_{smooth}(\phi)
    \label{eq:unsup_loss}
\end{equation}

If we consider additional segmentation for training then the loss function gets modified as below equation \ref{eq:voxelmorph_total_loss} where \(\mathcal{L}_{seg}\) is the segmentation loss

\begin{equation}
    \mathcal{L}_a(f, m, s_f, s_m, \phi) = \mathcal{L}_{us}(f, m, \phi)  + \gamma\mathcal{L}_{seg}(s_f, s_m \circ \phi)
    \label{eq:voxelmorph_total_loss}
\end{equation}

\subsubsection{Evaluation} The model is evaluated using DICE score against the segmentation from the fixed image. Voxelmorph outperforms traditional techniques such as ANTS-Syn method. It obtains an average dice of 0.786 to that of \(0.776\). Below Fig \ref{fig:Voxelmorph Example Output} \cite{balakrishnan_voxelmorph_2019} shows the registration of sample volumes that highlights registered landmarks and the deformation field.

\begin{figure*}[!htb]\centering
    \centering
    \includegraphics[width=1.0\textwidth]{figs/voxelmorph_sample_image.png}
    \caption{Voxelmorph Example Output}
    \label{fig:Voxelmorph Example Output}
\end{figure*}

\subsubsection{Proposed Method} \label{proposed_method}
\subsubsection{Introduction}
Deep Learning based techniques have been applied successfully to tackle various complex medical image processing problems. Over the years, several image registration techniques have been proposed using deep learning. Deformable image registration techniques such as Voxelmorph \cite{balakrishnan_voxelmorph_2019} have been successful in capturing finer changes and providing smoother deformations. However, Voxelmorph, as well as ICNet \cite{zhang_inverse-consistent_2018} and FIRE \cite{Wang2019} do not explicitly encode global dependencies (i.e. overall anatomical view of the supplied image) and track large deformations. This research improves upon Voxelmorph by employing self-constructing graph network SCGNet \cite{Liu2020SelfConstructingGC} to encode semantics which can improve the learning process of the model and help the model to generalise better, multi-scale supervision to be able to work well in case of small as well as large deformations, and cycle consistency for making the deformations consistent.   

\subsubsection{Hypothesis}
The proposed method tries to capture global dependencies using SCGNet \cite{Liu2020SelfConstructingGC}, wherein encoded CNN features are used to find out semantics. We hypothesize that these dependencies could help the model to learn relationships even between two distantly located structures in the fixed and moving image or voxels of ventricles filled with CSF and helps generate better deformations. As mentioned earlier, SCGNet was able to find clusters of similar information in the image using latent space features. If the model knows about the landmarks then it would be helpful for improving the deformation field. 

\cite{Chatterjee2020DS6DL} uses multi-scale supervised UNet to perform segmentation of vessels. We apply the multi-scale supervision to handle different amount of deformations, where deformations are predicted and losses are calculated for both original image and a downsampled image. We hypothesise that deformations on downsampled image would cover for larger deformations while the deformations on original image would produce finer deformations. The multi-scale supervision also allows for faster convergence, brings stability in the training as there would be multiple channels through which gradients can flow.

An adopted version of the cycle consistency loss, inspired by \cite{Zhou2016LearningDC}, was employed to maintain consistent deformations. Cycle consistency helps to maintain flow correspondence between fixed and moving image thereby drastically reducing the number of possible deformation fields to achieve the same deformation .Regularisation of sharp deformation was also used to obtain smooth deformation fields and remove unrealistic transformation. 

\subsubsection{Method} Let \(f\), \(m\) be fixed and moving n-D images where they belong to domain \( \Omega \subset \mathbb{R}^n\). We use 3-D single channel grayscale scans from IXI dataset \cite{ixiwebsite} for training but the framework is applicable also for other dimensions. We apply preprocessing treatment such as bias field correction, skull stripping, affine registration and intensity normalization on both the images. Both the images are then downscaled by a factor of two to be fed as secondary input. The complete CNN SCGNet based model parameterizes the function \(G_\theta\) that calculates the deformation field \(\phi\)  given a pair of fixed \(f\) and moving \(m\) images. The deformation field will have n-channels as it has to represent displacement in each of the n-axes. If its a 3-D image then deformation field will have 3 channels where each channel represent displacement in x, y and z axes respectively.

Proposed network takes in fixed \(f\) and moving \(m\) image along with its downsampled counterparts \(f_d\) and \(m_d\) and computes deformation field \(\phi\) and \(\phi_d\). Both the pairs are passed through the network and corresponding deformation fields are then applied to \(m \circ \phi \) and \(m_d \circ \phi_d \). Spatial transformers are used to warp the moving image and a similarity metric is used to compare \(f\) with \(m\) and \(f_d\) with \(m_d\). Gradient descent is used to minimize the loss and find optimal parameter \(\hat{\theta}\). Fig \ref{fig:Multi Scale UNet Overview} describes overview of the proposed model.

\begin{figure}[!htb]\centering
    \centering
    \includegraphics[width=1.3\textwidth]{figs/mscgunet_overview.png}
    \caption{Multi Scale UNet Overview}
    \label{fig:Multi Scale UNet Overview}
\end{figure}

\subsubsection{Architecture} The fixed \(f\) and moving \(m\) images are concatenated to the dimensions of $2 \times 128 \times 128 \times 128$ similarly downsampled images are concatenated with combined dimension of $2 \times 64 \times 64 \times 64$. The model uses UNet like structure to encode and decode the image information. For encoding, it uses convolution with stride of 2 and activation LeakyReLU to downsample the image and learn relevant features. Encoder near the latent space learn more high level features, whilst encoder at the beginning learns low level features that acts as an image pyramid. The encoded information is fed into the latent space of the SCGNet, which first parameterise the encodings to latent embeddings with mean and standard deviation and derives the undirected graph through an inner product of latent embeddings. The output is then fed into a fully-connected graph convolution network (GCN) which attempts to learn semantics of the brain anatomy. The GCN output is upsampled through trilinear interpolation and supplied to a CNN decoder which takes in also input from the respective encoder as skip connections. Each decoder block scales up the spatial dimensions of the image and reduces the channels by a factor of \(2\). Skip connections help improve gradient back propagation and training convergence. It also supplies the corresponding encoder information that provides location information that would be missing from decoder. Fixed image \(f\) and \(f_d\) are concatenated to the UNet output to maintain contrast of the fixed image \cite{Dewey2019DeepHarmonyAD}. Finally, deformation fields are smoothed by convolution layers which helps learn deformation at finer scales. Fig \ref{fig:Multi Scale UNet with SCG Architecture} illustrates the model architecture.


\begin{figure}[!htb]\centering
    \centering
    \includegraphics[ width=1.11\textwidth]{figs/mscgnet_without_image_architecture.png}
    \caption{Multi Scale UNet with SCGNet Architecture}
    \label{fig:Multi Scale UNet with SCG Architecture}
\end{figure}


\subsubsection{Training Procedure} We use publicly available IXI dataset \cite{ixiwebsite} to demonstrate the registration. 1000 images are used for training. The images are preprocessed using ANTs \cite{brian_b_avants_nicholas_j_tustison_gang_song_and_james_c_gee_ants_nodate}. During preprocessing we apply skull stripping, bias field correction, intensity normalisation and affine registration on the images. Fixed \(f\) and moving \(m\)  images were downsampled, the fixed \(f\) and moving \(m\) original images were concatenated and sent as an input to the network. Network processed the images and provides deformation fields at both original and downsampled scale. This is applied on both original, downsampled moving image and compared with both the fixed images. This process is repeated for the same image pair by swapping fixed and moving images. Finally both pair of losses equation \ref{eq:total_mscgunet_loss} are added up and back propagated through the network. Similarity measure Normalised Cross Correlation NCC and Normalised Mutual Information  NMI\( l_{sim}  \)were used for intramodal and intermodal registration for training. Smoothness loss \(l_{sm}\) \cite{Horn1981DeterminingOF} acts as regularise that penalises sharp deformations and SCG loss \(l_{scg}\) helps to learn similar features in the brain. \(\alpha , \beta\) and \(\lambda\) are hyper parameters. We experiment using various hyper parameters and make ablations to the network to measure the impact of each component on the registration performance. We run the training process on 500 images for \(1000\) epochs with learning rate of \(3e-4\). The hyper parameters \(\alpha\) and \(\alpha_d\) are set to \(-1.2\) and \(-0.6\), \(\beta\) and \(\beta_d\) are set to \(0.5\) and \(0.25\) and \(\lambda\) is \(5\). We achieve the best performance using these hyper parameters for the combination of dataset, preprocessing and the model.

\begin{equation}
l_{total} =  \alpha(l_{sim_{f->m}} + l_{sim_{m->f}})  + \alpha_d  (l_{sim_{f_d->m_d}} + l_{sim_{m_d->f_d}})  + 

\beta(l_{sm_{f->m}} + l_{sm_{m->f}})  + \beta_d(l_{sm_{f_d->m_d}} + l_{sm_{m_d->f_d}})  +

\lambda( l_{scg_{f->m}} + l_{scg_{m->f}} )  

\label{eq:total_mscgunet_loss}
\end{equation}

\begin{table*}[htb!]
    \centering
    \small
    \addtolength{\tabcolsep}{-1pt}
    \caption{Statistical T Test performed across Algorithms for Intramodal Evaluation with fixed and moving pairs flipped against original set of fixed and moving pairs }
    \label{tab:Algorithm_evaluation_pipeline_1_T_Test}
  \begin{tabular}{c  c  c  c  c  c  c}
    \toprule
    \multirow{2}{*}{Algorithm} &
      \multicolumn{5}{c}{Inverse Pairs (p values)} \\
      & {SSIM} & PCC & {Dice Score} & MSE & KL Distance \\
      \midrule
    Ants(SyN) & 0.8780 & 0.1248 &  0.6000 & 0.0010 & 0.1586\\
    ADMIR & 0 & 0  & 0.0015 & 0.311 & 0.0890\\ 
    RMSPROP & 0.6261 & 0.7588  & 0.0497 & 0.6783 & 0.9703\\ 
    VoxelMorph & 0 &  0 & 0.0016 & 0.0020 & 0.3630 \\
    MICDIR & 0.8221 & 0.1845 & 0.4893 & 0.5543 & 0.1353
 \\
    \bottomrule
  \end{tabular}
\end{table*}


\begin{table*}[htb!]
    \centering
    \small
    \addtolength{\tabcolsep}{-1pt}
    \caption{Statistical T Test performed between MICDIR and other Algorithms for Intramodal Evaluation with fixed and moving pairs flipped}
    \label{tab:MICDIR_evaluation_pipeline_1_T_Test}
  \begin{tabular}{c  c  c  c  c  c  c}
    \toprule
    \multirow{2}{*}{Algorithm} &
      \multicolumn{5}{c}{MICDIR (p values)} \\
      & {SSIM} & PCC & {Dice Score} & MSE & KL Distance \\
      \midrule
    Ants(SyN) & 0 & 0 &  0 & 0 & 0.3871\\
    ADMIR & 0 & 0  & 0 & 0.027 & 0.898\\ 
    RMSPROP & 0 & 0  & 0.0026 & 0 & 0.611\\ 
    VoxelMorph & 0 &  0 & 0 & 0 & 0.611 \\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{table*}[htb!]
    \centering
    \small
    \addtolength{\tabcolsep}{-1pt}
    \caption{Statistical T Test performed between MICDIR and other Algorithms for Intramodal Evaluation with fixed and moving pairs flipped}
    \label{tab:MICDIR_evaluation_pipeline_1_T_Test}
  \begin{tabular}{c  c  c  c  c  c  c}
    \toprule
    \multirow{2}{*}{Algorithm} &
      \multicolumn{5}{c}{MICDIR (p values)} \\
      & {SSIM} & PCC & {Dice Score} & MSE & KL Distance \\
      \midrule
    Ants(SyN) & 0 & 0 &  0 & 0 & 0.3871\\
    ADMIR & 0 & 0  & 0 & 0.027 & 0.898\\ 
    RMSPROP & 0 & 0  & 0.0026 & 0 & 0.611\\ 
    VoxelMorph & 0 &  0 & 0 & 0 & 0.611 \\
    \bottomrule
  \end{tabular}
\end{table*}




